Context Aware Nonnegative Matrix Factorization Clustering

In this article we propose a method to refine the clustering results obtained with the nonnegative matrix factorization (NMF) technique, imposing consistency constraints on the final labeling of the data. The research community focused its effort on the initialization and on the optimization part of this method, without paying attention to the final cluster assignments. We propose a game theoretic framework in which each object to be clustered is represented as a player, which has to choose its cluster membership. The information obtained with NMF is used to initialize the strategy space of the players and a weighted graph is used to model the interactions among the players. These interactions allow the players to choose a cluster which is coherent with the clusters chosen by similar players, a property which is not guaranteed by NMF, since it produces a soft clustering of the data. The results on common benchmarks show that our model is able to improve the performances of many NMF formulations.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> accuracy_sv_100.tex <==
\begin{table*}[tb] \centering \label{tab:results} \caption{Performance at 100 iteration for SV Method. Mean Loss(-0.17111  -0.0094444) Mean Gain(2.5603      2.2819).} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMFS & NNDSVD & SymNMF+GT & NMF+GT & NMFS+GT & NNDSVD+GT \\ \hline
NIPS & 0.46203 & \textbf{0.42571} & 0.46498 & 0.47406 & \textbf{0.48302} (+2.1\%) & 0.42465(--0.11\%) & \textbf{0.48479} (+1.98\%) & \textbf{0.50943} (+3.54\%) \\ \hline
NIPS TFIDF NP & 0.37927 & \textbf{0.39634} & 0.3837 & 0.46563 & \textbf{0.41452} (+3.53\%) & 0.39035(--0.6\%) & \textbf{0.40743} (+2.37\%) & \textbf{0.50333} (+3.77\%) \\ \hline
Reuters & 0.51725 & 0.32165 & 0.51587 & 0.40284 & \textbf{0.52804} (+1.08\%) & \textbf{0.40119} (+7.95\%) & \textbf{0.52479} (+0.89\%) & \textbf{0.42681} (+2.4\%) \\ \hline
ReutersNP & 0.32443 & 0.22152 & 0.33876 & 0.27664 & \textbf{0.36306} (+3.86\%) & \textbf{0.28151} (+6\%) & \textbf{0.37786} (+3.91\%) & \textbf{0.33869} (+6.21\%) \\ \hline
RCV1 & \textbf{0.29206} & 0.38323 & \textbf{0.29765} & \textbf{0.28467} & 0.28935(--0.27\%) & \textbf{0.3874} (+0.42\%) & 0.29662(--0.1\%) & 0.27644(--0.82\%) \\ \hline
PIE-Expr & 0.85366 & 0.7847 & 0.6306 & \textbf{0.55} & \textbf{0.86422} (+1.06\%) & \textbf{0.78858} (+0.39\%) & \textbf{0.71724} (+8.66\%) & 0.52306(--2.69\%) \\ \hline
ORL & 0.77575 & 0.4645 & 0.76963 & 0.65275 & \textbf{0.81138} (+3.56\%) & \textbf{0.60825} (+14.38\%) & \textbf{0.804} (+3.44\%) & \textbf{0.71} (+5.73\%) \\ \hline
COIL-20 & 0.72674 & 0.47799 & 0.73858 & \textbf{0.67354} & \textbf{0.72944} (+0.27\%) & \textbf{0.50667} (+2.87\%) & \textbf{0.74125} (+0.27\%) & 0.67188(--0.17\%) \\ \hline
ExtYaleB & \textbf{0.23521} & 0.19444 & \textbf{0.23698} & 0.22885 & 0.22795(--0.73\%) & \textbf{0.19665} (+0.22\%) & 0.23028(--0.67\%) & \textbf{0.24193} (+1.31\%) \\ \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMFS & NNDSVD & SymNMF+GT & NMF+GT & NMFS+GT & NNDSVD+GT \\ \hline
NIPS & 0.38518 & 0.37529 & 0.38828 & 0.38766 & \textbf{0.40521} (+2\%) & \textbf{0.38575} (+1.05\%) & \textbf{0.40263} (+1.43\%) & \textbf{0.39943} (+1.18\%) \\ \hline
NIPS TFIDF NP & 0.38698 & 0.40133 & 0.39276 & 0.38777 & \textbf{0.41844} (+3.15\%) & \textbf{0.40594} (+0.46\%) & \textbf{0.41216} (+1.94\%) & \textbf{0.42096} (+3.32\%) \\ \hline
Reuters & 0.5017 & 0.45088 & 0.50456 & \textbf{0.42671} & \textbf{0.50983} (+0.81\%) & \textbf{0.49025} (+3.94\%) & \textbf{0.51122} (+0.67\%) & 0.42493(--0.18\%) \\ \hline
ReutersNP & 0.51655 & 0.44177 & 0.51801 & 0.48772 & \textbf{0.52481} (+0.83\%) & \textbf{0.49712} (+5.53\%) & \textbf{0.52713} (+0.91\%) & \textbf{0.49281} (+0.51\%) \\ \hline
RCV1 & 0.40629 & 0.51012 & 0.40391 & \textbf{0.40264} & \textbf{0.42206} (+1.58\%) & \textbf{0.5156} (+0.55\%) & \textbf{0.42003} (+1.61\%) & 0.4017(--0.09\%) \\ \hline
PIE-Expr & 0.96369 & 0.93386 & 0.90109 & 0.86546 & \textbf{0.97286} (+0.92\%) & \textbf{0.95534} (+2.15\%) & \textbf{0.9415} (+4.04\%) & \textbf{0.89436} (+2.89\%) \\ \hline
ORL & 0.88835 & 0.69107 & 0.8891 & 0.80838 & \textbf{0.9205} (+3.22\%) & \textbf{0.84399} (+15.29\%) & \textbf{0.91805} (+2.9\%) & \textbf{0.89215} (+8.38\%) \\ \hline
COIL-20 & 0.87079 & 0.61943 & 0.87712 & 0.82425 & \textbf{0.87547} (+0.47\%) & \textbf{0.66875} (+4.93\%) & \textbf{0.88315} (+0.6\%) & \textbf{0.83628} (+1.2\%) \\ \hline
ExtYaleB & 0.30796 & \textbf{0.35554} & 0.30938 & 0.28804 & \textbf{0.31283} (+0.49\%) & 0.35488(--0.07\%) & \textbf{0.31395} (+0.46\%) & \textbf{0.31544} (+2.74\%) \\ \hline
\end{tabular}
\end{table*}


==> icpr2016 arXiv/IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> icpr2016 arXiv/accuracy_sv_100.tex <==
\begin{table*}[tb] \centering \label{tab:results} \caption{Performance at 100 iteration for SV Method. Mean Loss(-0.17111  -0.0094444) Mean Gain(2.5603      2.2819).} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMFS & NNDSVD & SymNMF+GT & NMF+GT & NMFS+GT & NNDSVD+GT \\ \hline
NIPS & 0.46203 & \textbf{0.42571} & 0.46498 & 0.47406 & \textbf{0.48302} (+2.1\%) & 0.42465(--0.11\%) & \textbf{0.48479} (+1.98\%) & \textbf{0.50943} (+3.54\%) \\ \hline
NIPS TFIDF NP & 0.37927 & \textbf{0.39634} & 0.3837 & 0.46563 & \textbf{0.41452} (+3.53\%) & 0.39035(--0.6\%) & \textbf{0.40743} (+2.37\%) & \textbf{0.50333} (+3.77\%) \\ \hline
Reuters & 0.51725 & 0.32165 & 0.51587 & 0.40284 & \textbf{0.52804} (+1.08\%) & \textbf{0.40119} (+7.95\%) & \textbf{0.52479} (+0.89\%) & \textbf{0.42681} (+2.4\%) \\ \hline
ReutersNP & 0.32443 & 0.22152 & 0.33876 & 0.27664 & \textbf{0.36306} (+3.86\%) & \textbf{0.28151} (+6\%) & \textbf{0.37786} (+3.91\%) & \textbf{0.33869} (+6.21\%) \\ \hline
RCV1 & \textbf{0.29206} & 0.38323 & \textbf{0.29765} & \textbf{0.28467} & 0.28935(--0.27\%) & \textbf{0.3874} (+0.42\%) & 0.29662(--0.1\%) & 0.27644(--0.82\%) \\ \hline
PIE-Expr & 0.85366 & 0.7847 & 0.6306 & \textbf{0.55} & \textbf{0.86422} (+1.06\%) & \textbf{0.78858} (+0.39\%) & \textbf{0.71724} (+8.66\%) & 0.52306(--2.69\%) \\ \hline
ORL & 0.77575 & 0.4645 & 0.76963 & 0.65275 & \textbf{0.81138} (+3.56\%) & \textbf{0.60825} (+14.38\%) & \textbf{0.804} (+3.44\%) & \textbf{0.71} (+5.73\%) \\ \hline
COIL-20 & 0.72674 & 0.47799 & 0.73858 & \textbf{0.67354} & \textbf{0.72944} (+0.27\%) & \textbf{0.50667} (+2.87\%) & \textbf{0.74125} (+0.27\%) & 0.67188(--0.17\%) \\ \hline
ExtYaleB & \textbf{0.23521} & 0.19444 & \textbf{0.23698} & 0.22885 & 0.22795(--0.73\%) & \textbf{0.19665} (+0.22\%) & 0.23028(--0.67\%) & \textbf{0.24193} (+1.31\%) \\ \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMFS & NNDSVD & SymNMF+GT & NMF+GT & NMFS+GT & NNDSVD+GT \\ \hline
NIPS & 0.38518 & 0.37529 & 0.38828 & 0.38766 & \textbf{0.40521} (+2\%) & \textbf{0.38575} (+1.05\%) & \textbf{0.40263} (+1.43\%) & \textbf{0.39943} (+1.18\%) \\ \hline
NIPS TFIDF NP & 0.38698 & 0.40133 & 0.39276 & 0.38777 & \textbf{0.41844} (+3.15\%) & \textbf{0.40594} (+0.46\%) & \textbf{0.41216} (+1.94\%) & \textbf{0.42096} (+3.32\%) \\ \hline
Reuters & 0.5017 & 0.45088 & 0.50456 & \textbf{0.42671} & \textbf{0.50983} (+0.81\%) & \textbf{0.49025} (+3.94\%) & \textbf{0.51122} (+0.67\%) & 0.42493(--0.18\%) \\ \hline
ReutersNP & 0.51655 & 0.44177 & 0.51801 & 0.48772 & \textbf{0.52481} (+0.83\%) & \textbf{0.49712} (+5.53\%) & \textbf{0.52713} (+0.91\%) & \textbf{0.49281} (+0.51\%) \\ \hline
RCV1 & 0.40629 & 0.51012 & 0.40391 & \textbf{0.40264} & \textbf{0.42206} (+1.58\%) & \textbf{0.5156} (+0.55\%) & \textbf{0.42003} (+1.61\%) & 0.4017(--0.09\%) \\ \hline
PIE-Expr & 0.96369 & 0.93386 & 0.90109 & 0.86546 & \textbf{0.97286} (+0.92\%) & \textbf{0.95534} (+2.15\%) & \textbf{0.9415} (+4.04\%) & \textbf{0.89436} (+2.89\%) \\ \hline
ORL & 0.88835 & 0.69107 & 0.8891 & 0.80838 & \textbf{0.9205} (+3.22\%) & \textbf{0.84399} (+15.29\%) & \textbf{0.91805} (+2.9\%) & \textbf{0.89215} (+8.38\%) \\ \hline
COIL-20 & 0.87079 & 0.61943 & 0.87712 & 0.82425 & \textbf{0.87547} (+0.47\%) & \textbf{0.66875} (+4.93\%) & \textbf{0.88315} (+0.6\%) & \textbf{0.83628} (+1.2\%) \\ \hline
ExtYaleB & 0.30796 & \textbf{0.35554} & 0.30938 & 0.28804 & \textbf{0.31283} (+0.49\%) & 0.35488(--0.07\%) & \textbf{0.31395} (+0.46\%) & \textbf{0.31544} (+2.74\%) \\ \hline
\end{tabular}
\end{table*}


==> icpr2016 arXiv/performance_gain_balance.tex <==
\begin{table*}[tb] \centering \caption{My caption} \label{my-label} \begin{tabular}{ll|ll|ll|ll|ll|} \textbf{} &  & \multicolumn{2}{l|}{\textbf{SymNMF+GT}} & \multicolumn{2}{l|}{\textbf{NMF+GT}} & \multicolumn{2}{l|}{\textbf{NMFS+GT}} & \multicolumn{2}{l|}{\textbf{NNDSVD+GT}} \\ \multicolumn{1}{|l}{\textbf{Dataset}} & \textbf{\#Points} & \textbf{Gain}      & \textbf{\#Pts}     & \textbf{Gain}    & \textbf{\#Pts}    & \textbf{Gain}     & \textbf{\#Pts}    & \textbf{Gain}      & \textbf{\#Pts}     \\ \hline


==> icpr2016 arXiv/performance_gain_elem.tex <==
\begin{table*}[tb] \centering \caption{My caption} \label{my-label} \begin{tabular}{ll|ll|ll|ll|ll|} \textbf{} &  & \multicolumn{2}{l|}{\textbf{SymNMF+GT}} & \multicolumn{2}{l|}{\textbf{NMF+GT}} & \multicolumn{2}{l|}{\textbf{NMFS+GT}} & \multicolumn{2}{l|}{\textbf{NNDSVD+GT}} \\ \multicolumn{1}{|l}{\textbf{Dataset}} & \textbf{\#Points} & \textbf{Gain}      & \textbf{\#Pts}     & \textbf{Gain}    & \textbf{\#Pts}    & \textbf{Gain}     & \textbf{\#Pts}    & \textbf{Gain}      & \textbf{\#Pts}     \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+2.1\%} & 8.904 & -0.1\% & 0.424 & \textbf{+2\%} & 8.48 & \textbf{+3.5\%} & 14.84 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+3.6\%} & 16.236 & -0.6\% & 2.706 & \textbf{+2.3\%} & 10.373 & \textbf{+3.7\%} & 16.687 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+1.1\%} & 89.045 & \textbf{+7.9\%} & 639.505 & \textbf{+0.9\%} & 72.855 & \textbf{+2.4\%} & 194.28 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+3.9\%} & 337.506 & \textbf{+6\%} & 519.24 & \textbf{+3.9\%} & 337.506 & \textbf{+6.2\%} & 536.548 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & -0.3\% & 39.762 & \textbf{+0.4\%} & 53.016 & -0.1\% & 13.254 & -0.9\% & 119.286 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+0.4\%} & 54.928 & \textbf{+1.6\%} & 219.712 & \textbf{+0.3\%} & 41.196 & \textbf{+0.1\%} & 13.732 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+4\%} & 9.28 & \textbf{+2.6\%} & 6.032 & \textbf{+8.3\%} & 19.256 & -2.3\% & 5.336 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+3.5\%} & 14 & \textbf{+14.3\%} & 57.2 & \textbf{+3.4\%} & 13.6 & \textbf{+5.7\%} & 22.8 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.2\%} & 2.88 & \textbf{+2.9\%} & 41.76 & \textbf{+0.2\%} & 2.88 & -0.2\% & 2.88 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & -0.7\% & 17.129 & \textbf{+0.3\%} & 7.341 & -0.7\% & 17.129 & \textbf{+1.3\%} & 31.811 \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+2\%} & 8.48 & \textbf{+1.1\%} & 4.664 & \textbf{+1.5\%} & 6.36 & \textbf{+1.1\%} & 4.664 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+3.1\%} & 13.981 & \textbf{+0.5\%} & 2.255 & \textbf{+1.9\%} & 8.569 & \textbf{+3.3\%} & 14.883 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+0.8\%} & 64.76 & \textbf{+3.9\%} & 315.705 & \textbf{+0.6\%} & 48.57 & -0.2\% & 16.19 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+0.8\%} & 69.232 & \textbf{+5.5\%} & 475.97 & \textbf{+0.9\%} & 77.886 & \textbf{+0.5\%} & 43.27 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & \textbf{+1.6\%} & 212.064 & \textbf{+0.6\%} & 79.524 & \textbf{+1.6\%} & 212.064 & -0.1\% & 13.254 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+1.1\%} & 151.052 & \textbf{+2.1\%} & 288.372 & \textbf{+1.1\%} & 151.052 & \textbf{+0.9\%} & 123.588 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+1.8\%} & 4.176 & \textbf{+2\%} & 4.64 & \textbf{+4.1\%} & 9.512 & \textbf{+2.9\%} & 6.728 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+3.3\%} & 13.2 & \textbf{+15.3\%} & 61.2 & \textbf{+2.9\%} & 11.6 & \textbf{+8.4\%} & 33.6 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.4\%} & 5.76 & \textbf{+5\%} & 72 & \textbf{+0.6\%} & 8.64 & \textbf{+1.2\%} & 17.28 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & \textbf{+0.5\%} & 12.235 & -0.1\% & 2.447 & \textbf{+0.5\%} & 12.235 & \textbf{+2.7\%} & 66.069 \\ \hline
\end{tabular}\end{table*}


==> icpr2016 arXiv/performance_gain_elem_floor-1.tex <==
\begin{table*}[tb] \centering \caption{My caption} \label{my-label} \begin{tabular}{ll|ll|ll|ll|ll|} \textbf{} &  & \multicolumn{2}{l|}{\textbf{SymNMF+GT}} & \multicolumn{2}{l|}{\textbf{NMF+GT}} & \multicolumn{2}{l|}{\textbf{NMFS+GT}} & \multicolumn{2}{l|}{\textbf{NNDSVD+GT}} \\ \multicolumn{1}{|l}{\textbf{Dataset}} & \textbf{\#Points} & \textbf{Gain}      & \textbf{\#Pts}     & \textbf{Gain}    & \textbf{\#Pts}    & \textbf{Gain}     & \textbf{\#Pts}    & \textbf{Gain}      & \textbf{\#Pts}     \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+2.6\%} & 11.024 & \textbf{+0.5\%} & 2.12 & \textbf{+2.8\%} & 11.872 & \textbf{+3.5\%} & 14.84 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+2.8\%} & 12.628 & -1\% & 4.51 & \textbf{+2.3\%} & 10.373 & \textbf{+4\%} & 18.04 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+0.9\%} & 72.855 & \textbf{+6.9\%} & 558.555 & \textbf{+1.2\%} & 97.14 & \textbf{+2.4\%} & 194.28 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+3.7\%} & 320.198 & \textbf{+5.8\%} & 501.932 & \textbf{+3.6\%} & 311.544 & \textbf{+5.6\%} & 484.624 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & -0.3\% & 39.762 & \textbf{+0.3\%} & 39.762 & -0.1\% & 13.254 & -0.9\% & 119.286 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+0.4\%} & 54.928 & \textbf{+1.5\%} & 205.98 & \textbf{+0.4\%} & 54.928 & \textbf{+0.3\%} & 41.196 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+4\%} & 9.28 & \textbf{+1.9\%} & 4.408 & \textbf{+7.5\%} & 17.4 & -0.6\% & 1.392 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+2.7\%} & 10.8 & \textbf{+13.4\%} & 53.6 & \textbf{+2.5\%} & 10 & \textbf{+8.2\%} & 32.8 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.4\%} & 5.76 & \textbf{+2.1\%} & 30.24 & \textbf{+0.4\%} & 5.76 & \textbf{+0.2\%} & 2.88 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & -0.6\% & 14.682 & \textbf{+0.7\%} & 17.129 & -0.6\% & 14.682 & \textbf{+1\%} & 24.47 \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+1.6\%} & 6.784 & \textbf{+2.4\%} & 10.176 & \textbf{+1.7\%} & 7.208 & \textbf{+1.3\%} & 5.512 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+1.8\%} & 8.118 & \textbf{+0.7\%} & 3.157 & \textbf{+1.5\%} & 6.765 & \textbf{+3\%} & 13.53 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+0.7\%} & 56.665 & \textbf{+3.8\%} & 307.61 & \textbf{+0.6\%} & 48.57 & -0.1\% & 8.095 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+0.7\%} & 60.578 & \textbf{+5.1\%} & 441.354 & \textbf{+0.7\%} & 60.578 & \textbf{+0.3\%} & 25.962 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & \textbf{+1.5\%} & 198.81 & \textbf{+0.6\%} & 79.524 & \textbf{+1.5\%} & 198.81 & -0.1\% & 13.254 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+1.1\%} & 151.052 & \textbf{+2.2\%} & 302.104 & \textbf{+0.9\%} & 123.588 & \textbf{+0.9\%} & 123.588 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+1.6\%} & 3.712 & \textbf{+2\%} & 4.64 & \textbf{+4.3\%} & 9.976 & \textbf{+3.3\%} & 7.656 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+2.5\%} & 10 & \textbf{+15.1\%} & 60.4 & \textbf{+2.4\%} & 9.6 & \textbf{+8.1\%} & 32.4 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.5\%} & 7.2 & \textbf{+4.3\%} & 61.92 & \textbf{+0.6\%} & 8.64 & \textbf{+1.5\%} & 21.6 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & \textbf{+0.9\%} & 22.023 & \textbf{+0.9\%} & 22.023 & \textbf{+0.8\%} & 19.576 & \textbf{+2.6\%} & 63.622 \\ \hline
\end{tabular}\end{table*}


==> icpr2016 arXiv/performance_sv_100.tex <==
\begin{table*}[ht] \centering 
 \caption{Performance of GTNMF compared to several NMF approaches. The mean and std deviation of 20 runs are reported.} \label{tab:results}
 \begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l"l|l"l|l"l|l"l|l|} \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.385 ($\pm 0.011$) & \textbf{0.405} ($\pm 0.016$) & 0.375 ($\pm 0.022$) & \textbf{0.386} ($\pm 0.011$) & 0.388 ($\pm 0.006$) & \textbf{0.403} ($\pm 0.007$) & 0.388 & \textbf{0.399}   \\ \hline
NIPS & 0.387 ($\pm 0.007$) & \textbf{0.418} ($\pm 0.017$) & 0.401 ($\pm 0.016$) & \textbf{0.406} ($\pm 0.016$) & 0.393 ($\pm 0.008$) & \textbf{0.412} ($\pm 0.018$) & 0.388 & \textbf{0.421}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.502 ($\pm 0.014$) & \textbf{0.51} ($\pm 0.016$) & 0.451 ($\pm 0.026$) & \textbf{0.49} ($\pm 0.02$) & 0.505 ($\pm 0.014$) & \textbf{0.511} ($\pm 0.015$) & \textbf{0.427} & 0.425 \\ \hline
Reuters & 0.517 ($\pm 0.007$) & \textbf{0.525} ($\pm 0.006$) & 0.442 ($\pm 0.006$) & \textbf{0.497} ($\pm 0.003$) & 0.518 ($\pm 0.006$) & \textbf{0.527} ($\pm 0.005$) & 0.488 & \textbf{0.493}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 ($\pm 0.007$) & \textbf{0.422} ($\pm 0.007$) & 0.51 ($\pm 0.007$) & \textbf{0.516} ($\pm 0.005$) & 0.404 ($\pm 0.009$) & \textbf{0.42} ($\pm 0.01$) & \textbf{0.403} & 0.402 \\ \hline
RCV1 & 0.411 ($\pm 0.006$) & \textbf{0.422} ($\pm 0.006$) & 0.462 ($\pm 0.009$) & \textbf{0.483} ($\pm 0.007$) & 0.413 ($\pm 0.006$) & \textbf{0.424} ($\pm 0.006$) & 0.398 & \textbf{0.407}   \\ \hline
PIE-Expr & 0.95 ($\pm 0.004$) & \textbf{0.968} ($\pm 0.004$) & 0.939 ($\pm 0.008$) & \textbf{0.959} ($\pm 0.006$) & 0.89 ($\pm 0.005$) & \textbf{0.931} ($\pm 0.006$) & 0.86 & \textbf{0.889}   \\ \hline
ORL & 0.888 ($\pm 0.006$) & \textbf{0.921} ($\pm 0.006$) & 0.691 ($\pm 0.015$) & \textbf{0.844} ($\pm 0.014$) & 0.889 ($\pm 0.006$) & \textbf{0.918} ($\pm 0.004$) & 0.808 & \textbf{0.892}   \\ \hline
COIL-20 & 0.871 ($\pm 0.009$) & \textbf{0.875} ($\pm 0.012$) & 0.619 ($\pm 0.017$) & \textbf{0.669} ($\pm 0.016$) & 0.877 ($\pm 0.013$) & \textbf{0.883} ($\pm 0.013$) & 0.824 & \textbf{0.836}   \\ \hline
ExtYaleB & 0.308 ($\pm 0.005$) & \textbf{0.313} ($\pm 0.005$) & \textbf{0.356} ($\pm 0.006$) & 0.355($\pm 0.007$) & 0.309 ($\pm 0.007$) & \textbf{0.314} ($\pm 0.005$) & 0.288 & \textbf{0.315}   \\ \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.462 ($\pm 0.013$) & \textbf{0.483} ($\pm 0.016$) & \textbf{0.426} ($\pm 0.02$) & 0.425($\pm 0.014$) & 0.465 ($\pm 0.011$) & \textbf{0.485} ($\pm 0.017$) & 0.474 & \textbf{0.509}   \\ \hline
NIPS & 0.379 ($\pm 0.01$) & \textbf{0.415} ($\pm 0.037$) & \textbf{0.396} ($\pm 0.022$) & 0.39($\pm 0.018$) & 0.384 ($\pm 0.014$) & \textbf{0.407} ($\pm 0.031$) & 0.466 & \textbf{0.503}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.517 ($\pm 0.044$) & \textbf{0.528} ($\pm 0.043$) & 0.322 ($\pm 0.024$) & \textbf{0.401} ($\pm 0.026$) & 0.516 ($\pm 0.037$) & \textbf{0.525} ($\pm 0.037$) & 0.403 & \textbf{0.427}   \\ \hline
Reuters & 0.324 ($\pm 0.029$) & \textbf{0.363} ($\pm 0.032$) & 0.222 ($\pm 0.011$) & \textbf{0.282} ($\pm 0.02$) & 0.339 ($\pm 0.023$) & \textbf{0.378} ($\pm 0.024$) & 0.277 & \textbf{0.339}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.292} ($\pm 0.015$) & 0.289($\pm 0.014$) & 0.383 ($\pm 0.009$) & \textbf{0.387} ($\pm 0.01$) & \textbf{0.298} ($\pm 0.017$) & 0.297($\pm 0.017$) & \textbf{0.285} & 0.276 \\ \hline
RCV1 & 0.243 ($\pm 0.008$) & \textbf{0.247} ($\pm 0.008$) & 0.279 ($\pm 0.01$) & \textbf{0.295} ($\pm 0.011$) & 0.242 ($\pm 0.01$) & \textbf{0.245} ($\pm 0.011$) & 0.239 & \textbf{0.24}   \\ \hline
PIE-Expr & 0.81 ($\pm 0.021$) & \textbf{0.85} ($\pm 0.019$) & 0.783 ($\pm 0.023$) & \textbf{0.809} ($\pm 0.024$) & 0.617 ($\pm 0.019$) & \textbf{0.7} ($\pm 0.02$) & \textbf{0.536} & 0.513 \\ \hline
ORL & 0.776 ($\pm 0.017$) & \textbf{0.811} ($\pm 0.018$) & 0.465 ($\pm 0.019$) & \textbf{0.608} ($\pm 0.026$) & 0.77 ($\pm 0.013$) & \textbf{0.804} ($\pm 0.015$) & 0.653 & \textbf{0.71}   \\ \hline
COIL-20 & 0.727 ($\pm 0.036$) & \textbf{0.729} ($\pm 0.037$) & 0.478 ($\pm 0.023$) & \textbf{0.507} ($\pm 0.025$) & 0.739 ($\pm 0.046$) & \textbf{0.741} ($\pm 0.046$) & \textbf{0.674} & 0.672 \\ \hline
ExtYaleB & \textbf{0.235} ($\pm 0.008$) & 0.228($\pm 0.007$) & 0.194 ($\pm 0.007$) & \textbf{0.197} ($\pm 0.009$) & \textbf{0.237} ($\pm 0.012$) & 0.23($\pm 0.01$) & 0.229 & \textbf{0.242}   \\ \hline
 \end{tabular} \end{adjustbox}
 \end{table*}


==> icpr2016 arXiv/performance_sv_100_.tex <==
\begin{table*}[ht] \centering 
 \caption{Performance of GTNMF compared to several NMF approaches. The mean and std deviation of 20 runs are reported.} \label{tab:results}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.385 ($\pm 0.011$) & \textbf{0.405} ($\pm 0.016$) & 0.375 ($\pm 0.022$) & \textbf{0.386} ($\pm 0.011$) & 0.388 ($\pm 0.006$) & \textbf{0.403} ($\pm 0.007$) & 0.388 & \textbf{0.399}   \\ \hline
NIPS & 0.387 ($\pm 0.007$) & \textbf{0.418} ($\pm 0.017$) & 0.401 ($\pm 0.016$) & \textbf{0.406} ($\pm 0.016$) & 0.393 ($\pm 0.008$) & \textbf{0.412} ($\pm 0.018$) & 0.388 & \textbf{0.421}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.502 ($\pm 0.014$) & \textbf{0.51} ($\pm 0.016$) & 0.451 ($\pm 0.026$) & \textbf{0.49} ($\pm 0.02$) & 0.505 ($\pm 0.014$) & \textbf{0.511} ($\pm 0.015$) & \textbf{0.427} & 0.425 \\ \hline
Reuters & 0.517 ($\pm 0.007$) & \textbf{0.525} ($\pm 0.006$) & 0.442 ($\pm 0.006$) & \textbf{0.497} ($\pm 0.003$) & 0.518 ($\pm 0.006$) & \textbf{0.527} ($\pm 0.005$) & 0.488 & \textbf{0.493}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 ($\pm 0.007$) & \textbf{0.422} ($\pm 0.007$) & 0.51 ($\pm 0.007$) & \textbf{0.516} ($\pm 0.005$) & 0.404 ($\pm 0.009$) & \textbf{0.42} ($\pm 0.01$) & \textbf{0.403} & 0.402 \\ \hline
RCV1 & 0.411 ($\pm 0.006$) & \textbf{0.422} ($\pm 0.006$) & 0.462 ($\pm 0.009$) & \textbf{0.483} ($\pm 0.007$) & 0.413 ($\pm 0.006$) & \textbf{0.424} ($\pm 0.006$) & 0.398 & \textbf{0.407}   \\ \hline
PIE-Expr & 0.95 ($\pm 0.004$) & \textbf{0.968} ($\pm 0.004$) & 0.939 ($\pm 0.008$) & \textbf{0.959} ($\pm 0.006$) & 0.89 ($\pm 0.005$) & \textbf{0.931} ($\pm 0.006$) & 0.86 & \textbf{0.889}   \\ \hline
ORL & 0.888 ($\pm 0.006$) & \textbf{0.921} ($\pm 0.006$) & 0.691 ($\pm 0.015$) & \textbf{0.844} ($\pm 0.014$) & 0.889 ($\pm 0.006$) & \textbf{0.918} ($\pm 0.004$) & 0.808 & \textbf{0.892}   \\ \hline
COIL-20 & 0.871 ($\pm 0.009$) & \textbf{0.875} ($\pm 0.012$) & 0.619 ($\pm 0.017$) & \textbf{0.669} ($\pm 0.016$) & 0.877 ($\pm 0.013$) & \textbf{0.883} ($\pm 0.013$) & 0.824 & \textbf{0.836}   \\ \hline
ExtYaleB & 0.308 ($\pm 0.005$) & \textbf{0.313} ($\pm 0.005$) & \textbf{0.356} ($\pm 0.006$) & 0.355($\pm 0.007$) & 0.309 ($\pm 0.007$) & \textbf{0.314} ($\pm 0.005$) & 0.288 & \textbf{0.315}   \\ \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.462 ($\pm 0.013$) & \textbf{0.483} ($\pm 0.016$) & \textbf{0.426} ($\pm 0.02$) & 0.425($\pm 0.014$) & 0.465 ($\pm 0.011$) & \textbf{0.485} ($\pm 0.017$) & 0.474 & \textbf{0.509}   \\ \hline
NIPS & 0.379 ($\pm 0.01$) & \textbf{0.415} ($\pm 0.037$) & \textbf{0.396} ($\pm 0.022$) & 0.39($\pm 0.018$) & 0.384 ($\pm 0.014$) & \textbf{0.407} ($\pm 0.031$) & 0.466 & \textbf{0.503}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.517 ($\pm 0.044$) & \textbf{0.528} ($\pm 0.043$) & 0.322 ($\pm 0.024$) & \textbf{0.401} ($\pm 0.026$) & 0.516 ($\pm 0.037$) & \textbf{0.525} ($\pm 0.037$) & 0.403 & \textbf{0.427}   \\ \hline
Reuters & 0.324 ($\pm 0.029$) & \textbf{0.363} ($\pm 0.032$) & 0.222 ($\pm 0.011$) & \textbf{0.282} ($\pm 0.02$) & 0.339 ($\pm 0.023$) & \textbf{0.378} ($\pm 0.024$) & 0.277 & \textbf{0.339}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.292} ($\pm 0.015$) & 0.289($\pm 0.014$) & 0.383 ($\pm 0.009$) & \textbf{0.387} ($\pm 0.01$) & \textbf{0.298} ($\pm 0.017$) & 0.297($\pm 0.017$) & \textbf{0.285} & 0.276 \\ \hline
RCV1 & 0.243 ($\pm 0.008$) & \textbf{0.247} ($\pm 0.008$) & 0.279 ($\pm 0.01$) & \textbf{0.295} ($\pm 0.011$) & 0.242 ($\pm 0.01$) & \textbf{0.245} ($\pm 0.011$) & 0.239 & \textbf{0.24}   \\ \hline
PIE-Expr & 0.81 ($\pm 0.021$) & \textbf{0.85} ($\pm 0.019$) & 0.783 ($\pm 0.023$) & \textbf{0.809} ($\pm 0.024$) & 0.617 ($\pm 0.019$) & \textbf{0.7} ($\pm 0.02$) & \textbf{0.536} & 0.513 \\ \hline
ORL & 0.776 ($\pm 0.017$) & \textbf{0.811} ($\pm 0.018$) & 0.465 ($\pm 0.019$) & \textbf{0.608} ($\pm 0.026$) & 0.77 ($\pm 0.013$) & \textbf{0.804} ($\pm 0.015$) & 0.653 & \textbf{0.71}   \\ \hline
COIL-20 & 0.727 ($\pm 0.036$) & \textbf{0.729} ($\pm 0.037$) & 0.478 ($\pm 0.023$) & \textbf{0.507} ($\pm 0.025$) & 0.739 ($\pm 0.046$) & \textbf{0.741} ($\pm 0.046$) & \textbf{0.674} & 0.672 \\ \hline
ExtYaleB & \textbf{0.235} ($\pm 0.008$) & 0.228($\pm 0.007$) & 0.194 ($\pm 0.007$) & \textbf{0.197} ($\pm 0.009$) & \textbf{0.237} ($\pm 0.012$) & 0.23($\pm 0.01$) & 0.229 & \textbf{0.242}   \\ \hline
 \end{tabular}
 \end{table*}


==> icpr2016 arXiv/performance_sv_100_floor_log.tex <==
\begin{table*}[tb] \centering \label{tab:results} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.464 ($\pm 0.017$) & \textbf{0.49} ($\pm 0.019$) & 0.429 ($\pm 0.022$) & \textbf{0.434} ($\pm 0.02$) & 0.467 ($\pm 0.013$) & \textbf{0.495} ($\pm 0.014$) & 0.474 & \textbf{0.509}   \\ \hline
NIPS & 0.381 ($\pm 0.012$) & \textbf{0.409} ($\pm 0.032$) & \textbf{0.4} ($\pm 0.015$) & 0.39($\pm 0.011$) & 0.38 ($\pm 0.013$) & \textbf{0.403} ($\pm 0.034$) & 0.466 & \textbf{0.506}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.522 ($\pm 0.049$) & \textbf{0.531} ($\pm 0.051$) & 0.339 ($\pm 0.033$) & \textbf{0.408} ($\pm 0.032$) & 0.502 ($\pm 0.058$) & \textbf{0.514} ($\pm 0.052$) & 0.403 & \textbf{0.427}   \\ \hline
Reuters & 0.33 ($\pm 0.021$) & \textbf{0.367} ($\pm 0.021$) & 0.222 ($\pm 0.008$) & \textbf{0.28} ($\pm 0.015$) & 0.341 ($\pm 0.018$) & \textbf{0.377} ($\pm 0.02$) & 0.277 & \textbf{0.333}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.294} ($\pm 0.014$) & 0.291($\pm 0.014$) & 0.384 ($\pm 0.012$) & \textbf{0.387} ($\pm 0.013$) & \textbf{0.297} ($\pm 0.012$) & 0.296($\pm 0.012$) & \textbf{0.285} & 0.276 \\ \hline
PIE-Expr & 0.809 ($\pm 0.027$) & \textbf{0.849} ($\pm 0.025$) & 0.791 ($\pm 0.02$) & \textbf{0.81} ($\pm 0.023$) & 0.622 ($\pm 0.018$) & \textbf{0.697} ($\pm 0.025$) & \textbf{0.536} & 0.53 \\ \hline
ORL & 0.775 ($\pm 0.017$) & \textbf{0.802} ($\pm 0.015$) & 0.456 ($\pm 0.019$) & \textbf{0.59} ($\pm 0.022$) & 0.776 ($\pm 0.015$) & \textbf{0.801} ($\pm 0.017$) & 0.653 & \textbf{0.735}   \\ \hline
COIL-20 & 0.716 ($\pm 0.052$) & \textbf{0.72} ($\pm 0.052$) & 0.476 ($\pm 0.028$) & \textbf{0.497} ($\pm 0.027$) & 0.745 ($\pm 0.046$) & \textbf{0.749} ($\pm 0.047$) & 0.669 & \textbf{0.671}   \\ \hline
ExtYaleB & \textbf{0.237} ($\pm 0.013$) & 0.231($\pm 0.011$) & 0.195 ($\pm 0.008$) & \textbf{0.202} ($\pm 0.009$) & \textbf{0.238} ($\pm 0.01$) & 0.232($\pm 0.009$) & 0.229 & \textbf{0.239}   \\ \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.386 ($\pm 0.012$) & \textbf{0.402} ($\pm 0.012$) & 0.374 ($\pm 0.026$) & \textbf{0.398} ($\pm 0.016$) & 0.388 ($\pm 0.006$) & \textbf{0.405} ($\pm 0.011$) & 0.388 & \textbf{0.401}   \\ \hline
NIPS & 0.389 ($\pm 0.009$) & \textbf{0.407} ($\pm 0.009$) & 0.404 ($\pm 0.015$) & \textbf{0.411} ($\pm 0.012$) & 0.388 ($\pm 0.009$) & \textbf{0.403} ($\pm 0.013$) & 0.388 & \textbf{0.418}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.499 ($\pm 0.017$) & \textbf{0.506} ($\pm 0.019$) & 0.456 ($\pm 0.02$) & \textbf{0.494} ($\pm 0.016$) & 0.495 ($\pm 0.019$) & \textbf{0.501} ($\pm 0.018$) & \textbf{0.427} & 0.426 \\ \hline
Reuters & 0.518 ($\pm 0.006$) & \textbf{0.525} ($\pm 0.005$) & 0.442 ($\pm 0.006$) & \textbf{0.493} ($\pm 0.004$) & 0.52 ($\pm 0.007$) & \textbf{0.527} ($\pm 0.006$) & 0.488 & \textbf{0.491}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 ($\pm 0.01$) & \textbf{0.421} ($\pm 0.01$) & 0.511 ($\pm 0.006$) & \textbf{0.517} ($\pm 0.006$) & 0.404 ($\pm 0.012$) & \textbf{0.419} ($\pm 0.011$) & \textbf{0.403} & 0.402 \\ \hline
PIE-Expr & 0.951 ($\pm 0.007$) & \textbf{0.967} ($\pm 0.005$) & 0.941 ($\pm 0.007$) & \textbf{0.961} ($\pm 0.005$) & 0.889 ($\pm 0.005$) & \textbf{0.932} ($\pm 0.006$) & 0.861 & \textbf{0.894}   \\ \hline
ORL & 0.889 ($\pm 0.007$) & \textbf{0.914} ($\pm 0.004$) & 0.682 ($\pm 0.017$) & \textbf{0.833} ($\pm 0.014$) & 0.89 ($\pm 0.005$) & \textbf{0.914} ($\pm 0.005$) & 0.808 & \textbf{0.889}   \\ \hline
COIL-20 & 0.87 ($\pm 0.015$) & \textbf{0.875} ($\pm 0.016$) & 0.62 ($\pm 0.017$) & \textbf{0.663} ($\pm 0.015$) & 0.878 ($\pm 0.009$) & \textbf{0.884} ($\pm 0.011$) & 0.82 & \textbf{0.835}   \\ \hline
ExtYaleB & 0.306 ($\pm 0.008$) & \textbf{0.315} ($\pm 0.006$) & 0.356 ($\pm 0.008$) & \textbf{0.365} ($\pm 0.008$) & 0.311 ($\pm 0.008$) & \textbf{0.319} ($\pm 0.005$) & 0.288 & \textbf{0.314}   \\ \hline
 \end{tabular}
 \caption{Performance of the GT-NMF compared to other approaches.}
 \end{table*}


==> icpr2016 arXiv/performance_sv_100_sv_floor_log.tex <==
\begin{table*}[tb] \centering \label{tab:results} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.464 & \textbf{0.49} (+2.6\%) & 0.429 & \textbf{0.434} (+0.5\%) & 0.467 & \textbf{0.495} (+2.8\%) & 0.474 & \textbf{0.509} (+3.5\%) \\ \hline
NIPS & 0.381 & \textbf{0.409} (+2.8\%) & \textbf{0.4} & 0.39(--1\%) & 0.38 & \textbf{0.403} (+2.3\%) & 0.466 & \textbf{0.506} (+4\%) \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.522 & \textbf{0.531} (+0.9\%) & 0.339 & \textbf{0.408} (+6.9\%) & 0.502 & \textbf{0.514} (+1.2\%) & 0.403 & \textbf{0.427} (+2.4\%) \\ \hline
Reuters & 0.33 & \textbf{0.367} (+3.7\%) & 0.222 & \textbf{0.28} (+5.8\%) & 0.341 & \textbf{0.377} (+3.6\%) & 0.277 & \textbf{0.333} (+5.6\%) \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.294} & 0.291(--0.3\%) & 0.384 & \textbf{0.387} (+0.3\%) & \textbf{0.297} & 0.296(--0.1\%) & \textbf{0.285} & 0.276(--0.9\%) \\ \hline
PIE-Expr & 0.809 & \textbf{0.849} (+4\%) & 0.791 & \textbf{0.81} (+1.9\%) & 0.622 & \textbf{0.697} (+7.5\%) & \textbf{0.536} & 0.53(--0.6\%) \\ \hline
ORL & 0.775 & \textbf{0.802} (+2.7\%) & 0.456 & \textbf{0.59} (+13.4\%) & 0.776 & \textbf{0.801} (+2.5\%) & 0.653 & \textbf{0.735} (+8.2\%) \\ \hline
COIL-20 & 0.716 & \textbf{0.72} (+0.4\%) & 0.476 & \textbf{0.497} (+2.1\%) & 0.745 & \textbf{0.749} (+0.4\%) & 0.669 & \textbf{0.671} (+0.2\%) \\ \hline
ExtYaleB & \textbf{0.237} & 0.231(--0.6\%) & 0.195 & \textbf{0.202} (+0.7\%) & \textbf{0.238} & 0.232(--0.6\%) & 0.229 & \textbf{0.239} (+1\%) \\ \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.386 & \textbf{0.402} (+1.6\%) & 0.374 & \textbf{0.398} (+2.4\%) & 0.388 & \textbf{0.405} (+1.7\%) & 0.388 & \textbf{0.401} (+1.3\%) \\ \hline
NIPS & 0.389 & \textbf{0.407} (+1.8\%) & 0.404 & \textbf{0.411} (+0.7\%) & 0.388 & \textbf{0.403} (+1.5\%) & 0.388 & \textbf{0.418} (+3\%) \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.499 & \textbf{0.506} (+0.7\%) & 0.456 & \textbf{0.494} (+3.8\%) & 0.495 & \textbf{0.501} (+0.6\%) & \textbf{0.427} & 0.426(--0.1\%) \\ \hline
Reuters & 0.518 & \textbf{0.525} (+0.7\%) & 0.442 & \textbf{0.493} (+5.1\%) & 0.52 & \textbf{0.527} (+0.7\%) & 0.488 & \textbf{0.491} (+0.3\%) \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 & \textbf{0.421} (+1.5\%) & 0.511 & \textbf{0.517} (+0.6\%) & 0.404 & \textbf{0.419} (+1.5\%) & \textbf{0.403} & 0.402(--0.1\%) \\ \hline
PIE-Expr & 0.951 & \textbf{0.967} (+1.6\%) & 0.941 & \textbf{0.961} (+2\%) & 0.889 & \textbf{0.932} (+4.3\%) & 0.861 & \textbf{0.894} (+3.3\%) \\ \hline
ORL & 0.889 & \textbf{0.914} (+2.5\%) & 0.682 & \textbf{0.833} (+15.1\%) & 0.89 & \textbf{0.914} (+2.4\%) & 0.808 & \textbf{0.889} (+8.1\%) \\ \hline
COIL-20 & 0.87 & \textbf{0.875} (+0.5\%) & 0.62 & \textbf{0.663} (+4.3\%) & 0.878 & \textbf{0.884} (+0.6\%) & 0.82 & \textbf{0.835} (+1.5\%) \\ \hline
ExtYaleB & 0.306 & \textbf{0.315} (+0.9\%) & 0.356 & \textbf{0.365} (+0.9\%) & 0.311 & \textbf{0.319} (+0.8\%) & 0.288 & \textbf{0.314} (+2.6\%) \\ \hline
 \end{tabular}
 \caption{Performance at 100 iteration for SV Method. Mean Loss(-0.11389  -0.0055556) Mean Gain(2.6083      2.2472).}
 \end{table*}


==> icpr2016 arXiv/seba.tex <==
%\section{Similarity Matrix construction}\label{sec:smc}
%
%The same pipeline of \cite{kuang2015symnmf} has been used to construct the similarity matrix, this has been done to fairly compare the performances at the end. Given a feature matrix of $n \times m$ data in which $n$ is the number of points and $m$ the size of the feature, each point became a vertex and the weight of the edges $e_{ij}$ are computed in the following 3 steps:\\
%
%\emph{1. Construct a complete graph}: If the dataset $X$ is textual each row is normalized to have unit 2-norm and $e_{i,j}={x_i}^Tx_j$ are the cosine distance of point $i$ and $j$. If $X$ is made of images each feature (column) is first normalized by its maximum value to lie in $[0,1]$ and then the weight are $e_{i,j}=\exp\{- \frac{||x_i-x_j||}{\sigma_i\sigma_j}\}$ where $\sigma_i=||x_i-\hat{x_i}||$ is a scaling parameter and $\hat{x_i}$ is the 7-th nearest neighbors, as suggested in \cite{Zelnik-manor04self-tuningspectral}. In all cases $e_{ii}=0$.\\
%
%\emph{2. Graph sparsification}: Only the edges connecting $q$ neighbors are kept. The parameter $q$ is set accordingly to \cite{Luxburg2007} $q=\floor{log_2(n)}+1$, let $N(i)=\{ j \mbox{ s.t. } x_j \in q\mbox{-NN of } i \}$. The weight on the edges are $\hat{e}_{ij}=e_{ij}$ if $i \in N(j) \mbox{ or } j\in N(i)$ and $\hat{e}_{ij}=0$ otherwise.\\
%
%\emph{3. Similarity Matrix}: the same normalization of normalized-cut has been applied on the sparse graph obtaining the final matrix $A_{ij}=\hat{e}_{ij}\sqrt{d_i}\sqrt{d_j}$ where $d_i=\sum_{s=1}^n{\hat{e}_{is}}$.
%



\section{Adaptive auto-tuning} When constructing the payoff matrix $A$ for the
game dynamics the same procedure of Sec \ref{sec:smc} is used with the only,
important, difference on how the parameter $q$ is chosen. The assumption here is
that the clustering results obtained via NMF provides a good insight on the size
of the final clusters and this information can be used to select the number of
$q$. The rationale is that clusters induces games in which the number of players
is in the order of the number of the elements within them (small clusters let a
small number of players to ply while bigger clusters let a bigger number of
players to play). In this context having a fixed $q$ all the clusters may lead
to have players belonging to small cluster that plays with a bigger number of
opponents. The idea to solve this problem by using the same idea of
\cite{Luxburg2007} applied in a local context having a variable $q$ for all
clusters obtained via NMF. Given a point $i$ and its clustering membership $C$
from NMF ($i \in C$), the number of neighbors used to construct the similarity
matrix is related to the expected number of points in the cluster $C$. This
results in having a variable number of expected number of neighbors depending on
the clusters size $q_i= \floor{log(|C|)}+1$ where $|C|$ is the cardinality of
cluster $C$. This intuition have the following combinatorial counterpart: a
theoretical bound to prove the connectedness of a graph \cite{Luxburg2007} is
that a graph is connected if the number of neighbors of each node is
$k=\floor{log(n)}+1$. A cluster $C$ can be considered as a fully connected
subgraph and thus connected. Thus the number of neighbors of each element in the
cluster $C$ should be $k_C=\floor{log(|C|)}+1$ where $|C|$ is the number of
elements in the cluster otherwise the subgraph is not connected and thus is not
a cluster. 

\subsection{results analysis} A global analysis on the results obtained by the
GTNMF shown the efficancy of using this approach to refine the partitions
obtained by NMF and derivate methods. Despite the different settings
(textual/image datasets) the algorithm is able improve the NMI performance in
33/36 cases with a maximum gain of $\simeq 15.3\%$ (which is quite impressive)
and a maximum loss of 0.2\%. In terms of ACC on 27/36 cases the method improve
on previous results with a maximum gain of 14.3\% and loss of 2.3\%. The mean
gain for both NMI and ACC is $2.68\%$ and $2.30\%$ while the mean loss is in the
order of $0.16\%$ for the ACC and $0.01\%$ in the NMI (see Table
\ref{tab:results}). An almost constant gain in the NMI means, in practice, that
the algorithm is able to correctly relocate the points in the right cluster
after the NMF clustering. This is quite a good results if the gain is related to
the size of the dataset, i.e. a gain of $+1.6\%$ in RCV1 means that 212 elements
has been moved. Giving a closer look on the results one can notice that in some
cases the ACC and the NMI have opposite behavior in the sense that when there is
a drop in the ACC a gain is achieved in the NMI, this is quite normal and is
explained by the fact that the NMI provides hints on how good the data are
partitioned while the ACC counts only the correct assignment (ESEMPIO TOY DI
ROCCO), the opposite is indeed true as well. Checking more carefully the case in
which the performances are lower (PIE-Expr with NNDSVD+GT) this happens mainly
because the clusters are a lot (68) while the data per cluster is not constant
and rolls between 3 and 4, a small change in this dataset dramatically impact
the global performance.\\




For those dataset in which 

Giving a closer look on when the looses occurs one can notice that this happen
in deeper analysis on when the losses occur

==> icpr2016 arXiv/table_datasets.tex <==
\begin{table*}[] \centering \caption{Datasets description. \textsuperscript{$\bigstar$} = the dataset has been pruned as in \protect\cite{kuang2015symnmf}.} \label{tbl:datasets} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline Dataset & Type & Points & Features & Clusters & Balance & Mean Clust & Min Cl Size & Max Cl Size \\ \hline
NIPS\textsuperscript{$\bigstar$} & text & 424 & 17522 & 9 & 0.105 & 47.1 & 15 & 143 \\ \hline
NIPS & text & 451 & 17522 & 13 & 0.028 & 34.7 & 4 & 143 \\ \hline
Reuters\textsuperscript{$\bigstar$} & text & 8095 & 14143 & 20 & 0.011 & 404.8 & 42 & 3735 \\ \hline
Reuters & text & 8654 & 14333 & 65 & 0 & 133.1 & 1 & 3735 \\ \hline
RCV1\textsuperscript{$\bigstar$} & text & 13254 & 20478 & 40 & 0.028 & 331.4 & 45 & 1587 \\ \hline
RCV1 & text & 13732 & 20478 & 75 & 0.001 & 183.1 & 1 & 1587 \\ \hline
PIE-Expr & image & 232 & 4096 & 68 & 0.75 & 3.4 & 3 & 4 \\ \hline
ORL & image & 400 & 5796 & 40 & 1 & 10 & 10 & 10 \\ \hline
COIL-20 & image & 1440 & 4096 & 20 & 1 & 72 & 72 & 72 \\ \hline
ExtYaleB & image & 2447 & 3584 & 38 & 0.678 & 64.4 & 59 & 87 \\ \hline
\end{tabular}\end{table*}


==> performance_gain_balance.tex <==
\begin{table*}[tb] \centering \caption{My caption} \label{my-label} \begin{tabular}{ll|ll|ll|ll|ll|} \textbf{} &  & \multicolumn{2}{l|}{\textbf{SymNMF+GT}} & \multicolumn{2}{l|}{\textbf{NMF+GT}} & \multicolumn{2}{l|}{\textbf{NMFS+GT}} & \multicolumn{2}{l|}{\textbf{NNDSVD+GT}} \\ \multicolumn{1}{|l}{\textbf{Dataset}} & \textbf{\#Points} & \textbf{Gain}      & \textbf{\#Pts}     & \textbf{Gain}    & \textbf{\#Pts}    & \textbf{Gain}     & \textbf{\#Pts}    & \textbf{Gain}      & \textbf{\#Pts}     \\ \hline


==> performance_gain_elem.tex <==
\begin{table*}[tb] \centering \caption{My caption} \label{my-label} \begin{tabular}{ll|ll|ll|ll|ll|} \textbf{} &  & \multicolumn{2}{l|}{\textbf{SymNMF+GT}} & \multicolumn{2}{l|}{\textbf{NMF+GT}} & \multicolumn{2}{l|}{\textbf{NMFS+GT}} & \multicolumn{2}{l|}{\textbf{NNDSVD+GT}} \\ \multicolumn{1}{|l}{\textbf{Dataset}} & \textbf{\#Points} & \textbf{Gain}      & \textbf{\#Pts}     & \textbf{Gain}    & \textbf{\#Pts}    & \textbf{Gain}     & \textbf{\#Pts}    & \textbf{Gain}      & \textbf{\#Pts}     \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+2.1\%} & 8.904 & -0.1\% & 0.424 & \textbf{+2\%} & 8.48 & \textbf{+3.5\%} & 14.84 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+3.6\%} & 16.236 & -0.6\% & 2.706 & \textbf{+2.3\%} & 10.373 & \textbf{+3.7\%} & 16.687 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+1.1\%} & 89.045 & \textbf{+7.9\%} & 639.505 & \textbf{+0.9\%} & 72.855 & \textbf{+2.4\%} & 194.28 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+3.9\%} & 337.506 & \textbf{+6\%} & 519.24 & \textbf{+3.9\%} & 337.506 & \textbf{+6.2\%} & 536.548 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & -0.3\% & 39.762 & \textbf{+0.4\%} & 53.016 & -0.1\% & 13.254 & -0.9\% & 119.286 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+0.4\%} & 54.928 & \textbf{+1.6\%} & 219.712 & \textbf{+0.3\%} & 41.196 & \textbf{+0.1\%} & 13.732 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+4\%} & 9.28 & \textbf{+2.6\%} & 6.032 & \textbf{+8.3\%} & 19.256 & -2.3\% & 5.336 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+3.5\%} & 14 & \textbf{+14.3\%} & 57.2 & \textbf{+3.4\%} & 13.6 & \textbf{+5.7\%} & 22.8 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.2\%} & 2.88 & \textbf{+2.9\%} & 41.76 & \textbf{+0.2\%} & 2.88 & -0.2\% & 2.88 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & -0.7\% & 17.129 & \textbf{+0.3\%} & 7.341 & -0.7\% & 17.129 & \textbf{+1.3\%} & 31.811 \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+2\%} & 8.48 & \textbf{+1.1\%} & 4.664 & \textbf{+1.5\%} & 6.36 & \textbf{+1.1\%} & 4.664 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+3.1\%} & 13.981 & \textbf{+0.5\%} & 2.255 & \textbf{+1.9\%} & 8.569 & \textbf{+3.3\%} & 14.883 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+0.8\%} & 64.76 & \textbf{+3.9\%} & 315.705 & \textbf{+0.6\%} & 48.57 & -0.2\% & 16.19 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+0.8\%} & 69.232 & \textbf{+5.5\%} & 475.97 & \textbf{+0.9\%} & 77.886 & \textbf{+0.5\%} & 43.27 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & \textbf{+1.6\%} & 212.064 & \textbf{+0.6\%} & 79.524 & \textbf{+1.6\%} & 212.064 & -0.1\% & 13.254 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+1.1\%} & 151.052 & \textbf{+2.1\%} & 288.372 & \textbf{+1.1\%} & 151.052 & \textbf{+0.9\%} & 123.588 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+1.8\%} & 4.176 & \textbf{+2\%} & 4.64 & \textbf{+4.1\%} & 9.512 & \textbf{+2.9\%} & 6.728 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+3.3\%} & 13.2 & \textbf{+15.3\%} & 61.2 & \textbf{+2.9\%} & 11.6 & \textbf{+8.4\%} & 33.6 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.4\%} & 5.76 & \textbf{+5\%} & 72 & \textbf{+0.6\%} & 8.64 & \textbf{+1.2\%} & 17.28 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & \textbf{+0.5\%} & 12.235 & -0.1\% & 2.447 & \textbf{+0.5\%} & 12.235 & \textbf{+2.7\%} & 66.069 \\ \hline
\end{tabular}\end{table*}


==> performance_gain_elem_floor-1.tex <==
\begin{table*}[tb] \centering \caption{My caption} \label{my-label} \begin{tabular}{ll|ll|ll|ll|ll|} \textbf{} &  & \multicolumn{2}{l|}{\textbf{SymNMF+GT}} & \multicolumn{2}{l|}{\textbf{NMF+GT}} & \multicolumn{2}{l|}{\textbf{NMFS+GT}} & \multicolumn{2}{l|}{\textbf{NNDSVD+GT}} \\ \multicolumn{1}{|l}{\textbf{Dataset}} & \textbf{\#Points} & \textbf{Gain}      & \textbf{\#Pts}     & \textbf{Gain}    & \textbf{\#Pts}    & \textbf{Gain}     & \textbf{\#Pts}    & \textbf{Gain}      & \textbf{\#Pts}     \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+2.6\%} & 11.024 & \textbf{+0.5\%} & 2.12 & \textbf{+2.8\%} & 11.872 & \textbf{+3.5\%} & 14.84 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+2.8\%} & 12.628 & -1\% & 4.51 & \textbf{+2.3\%} & 10.373 & \textbf{+4\%} & 18.04 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+0.9\%} & 72.855 & \textbf{+6.9\%} & 558.555 & \textbf{+1.2\%} & 97.14 & \textbf{+2.4\%} & 194.28 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+3.7\%} & 320.198 & \textbf{+5.8\%} & 501.932 & \textbf{+3.6\%} & 311.544 & \textbf{+5.6\%} & 484.624 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & -0.3\% & 39.762 & \textbf{+0.3\%} & 39.762 & -0.1\% & 13.254 & -0.9\% & 119.286 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+0.4\%} & 54.928 & \textbf{+1.5\%} & 205.98 & \textbf{+0.4\%} & 54.928 & \textbf{+0.3\%} & 41.196 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+4\%} & 9.28 & \textbf{+1.9\%} & 4.408 & \textbf{+7.5\%} & 17.4 & -0.6\% & 1.392 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+2.7\%} & 10.8 & \textbf{+13.4\%} & 53.6 & \textbf{+2.5\%} & 10 & \textbf{+8.2\%} & 32.8 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.4\%} & 5.76 & \textbf{+2.1\%} & 30.24 & \textbf{+0.4\%} & 5.76 & \textbf{+0.2\%} & 2.88 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & -0.6\% & 14.682 & \textbf{+0.7\%} & 17.129 & -0.6\% & 14.682 & \textbf{+1\%} & 24.47 \\ \hline
\multicolumn{1}{|l}{NIPS \textsuperscript{$\bigstar$}}  & 424 & \textbf{+1.6\%} & 6.784 & \textbf{+2.4\%} & 10.176 & \textbf{+1.7\%} & 7.208 & \textbf{+1.3\%} & 5.512 \\ \hline
\multicolumn{1}{|l}{NIPS}  & 451 & \textbf{+1.8\%} & 8.118 & \textbf{+0.7\%} & 3.157 & \textbf{+1.5\%} & 6.765 & \textbf{+3\%} & 13.53 \\ \hline
\multicolumn{1}{|l}{Reuters \textsuperscript{$\bigstar$}}  & 8095 & \textbf{+0.7\%} & 56.665 & \textbf{+3.8\%} & 307.61 & \textbf{+0.6\%} & 48.57 & -0.1\% & 8.095 \\ \hline
\multicolumn{1}{|l}{Reuters}  & 8654 & \textbf{+0.7\%} & 60.578 & \textbf{+5.1\%} & 441.354 & \textbf{+0.7\%} & 60.578 & \textbf{+0.3\%} & 25.962 \\ \hline
\multicolumn{1}{|l}{RCV1 \textsuperscript{$\bigstar$}}  & 13254 & \textbf{+1.5\%} & 198.81 & \textbf{+0.6\%} & 79.524 & \textbf{+1.5\%} & 198.81 & -0.1\% & 13.254 \\ \hline
\multicolumn{1}{|l}{RCV1}  & 13732 & \textbf{+1.1\%} & 151.052 & \textbf{+2.2\%} & 302.104 & \textbf{+0.9\%} & 123.588 & \textbf{+0.9\%} & 123.588 \\ \hline
\multicolumn{1}{|l}{PIE-Expr}  & 232 & \textbf{+1.6\%} & 3.712 & \textbf{+2\%} & 4.64 & \textbf{+4.3\%} & 9.976 & \textbf{+3.3\%} & 7.656 \\ \hline
\multicolumn{1}{|l}{ORL}  & 400 & \textbf{+2.5\%} & 10 & \textbf{+15.1\%} & 60.4 & \textbf{+2.4\%} & 9.6 & \textbf{+8.1\%} & 32.4 \\ \hline
\multicolumn{1}{|l}{COIL-20}  & 1440 & \textbf{+0.5\%} & 7.2 & \textbf{+4.3\%} & 61.92 & \textbf{+0.6\%} & 8.64 & \textbf{+1.5\%} & 21.6 \\ \hline
\multicolumn{1}{|l}{ExtYaleB}  & 2447 & \textbf{+0.9\%} & 22.023 & \textbf{+0.9\%} & 22.023 & \textbf{+0.8\%} & 19.576 & \textbf{+2.6\%} & 63.622 \\ \hline
\end{tabular}\end{table*}


==> performance_sv_100_.tex <==
\begin{table*}[ht] \centering 
 \caption{Performance of GTNMF compared to several NMF approaches. The mean and std deviation of 20 runs are reported.} \label{tab:results}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.385 ($\pm 0.011$) & \textbf{0.405} ($\pm 0.016$) & 0.375 ($\pm 0.022$) & \textbf{0.386} ($\pm 0.011$) & 0.388 ($\pm 0.006$) & \textbf{0.403} ($\pm 0.007$) & 0.388 & \textbf{0.399}   \\ \hline
NIPS & 0.387 ($\pm 0.007$) & \textbf{0.418} ($\pm 0.017$) & 0.401 ($\pm 0.016$) & \textbf{0.406} ($\pm 0.016$) & 0.393 ($\pm 0.008$) & \textbf{0.412} ($\pm 0.018$) & 0.388 & \textbf{0.421}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.502 ($\pm 0.014$) & \textbf{0.51} ($\pm 0.016$) & 0.451 ($\pm 0.026$) & \textbf{0.49} ($\pm 0.02$) & 0.505 ($\pm 0.014$) & \textbf{0.511} ($\pm 0.015$) & \textbf{0.427} & 0.425 \\ \hline
Reuters & 0.517 ($\pm 0.007$) & \textbf{0.525} ($\pm 0.006$) & 0.442 ($\pm 0.006$) & \textbf{0.497} ($\pm 0.003$) & 0.518 ($\pm 0.006$) & \textbf{0.527} ($\pm 0.005$) & 0.488 & \textbf{0.493}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 ($\pm 0.007$) & \textbf{0.422} ($\pm 0.007$) & 0.51 ($\pm 0.007$) & \textbf{0.516} ($\pm 0.005$) & 0.404 ($\pm 0.009$) & \textbf{0.42} ($\pm 0.01$) & \textbf{0.403} & 0.402 \\ \hline
RCV1 & 0.411 ($\pm 0.006$) & \textbf{0.422} ($\pm 0.006$) & 0.462 ($\pm 0.009$) & \textbf{0.483} ($\pm 0.007$) & 0.413 ($\pm 0.006$) & \textbf{0.424} ($\pm 0.006$) & 0.398 & \textbf{0.407}   \\ \hline
PIE-Expr & 0.95 ($\pm 0.004$) & \textbf{0.968} ($\pm 0.004$) & 0.939 ($\pm 0.008$) & \textbf{0.959} ($\pm 0.006$) & 0.89 ($\pm 0.005$) & \textbf{0.931} ($\pm 0.006$) & 0.86 & \textbf{0.889}   \\ \hline
ORL & 0.888 ($\pm 0.006$) & \textbf{0.921} ($\pm 0.006$) & 0.691 ($\pm 0.015$) & \textbf{0.844} ($\pm 0.014$) & 0.889 ($\pm 0.006$) & \textbf{0.918} ($\pm 0.004$) & 0.808 & \textbf{0.892}   \\ \hline
COIL-20 & 0.871 ($\pm 0.009$) & \textbf{0.875} ($\pm 0.012$) & 0.619 ($\pm 0.017$) & \textbf{0.669} ($\pm 0.016$) & 0.877 ($\pm 0.013$) & \textbf{0.883} ($\pm 0.013$) & 0.824 & \textbf{0.836}   \\ \hline
ExtYaleB & 0.308 ($\pm 0.005$) & \textbf{0.313} ($\pm 0.005$) & \textbf{0.356} ($\pm 0.006$) & 0.355($\pm 0.007$) & 0.309 ($\pm 0.007$) & \textbf{0.314} ($\pm 0.005$) & 0.288 & \textbf{0.315}   \\ \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.462 ($\pm 0.013$) & \textbf{0.483} ($\pm 0.016$) & \textbf{0.426} ($\pm 0.02$) & 0.425($\pm 0.014$) & 0.465 ($\pm 0.011$) & \textbf{0.485} ($\pm 0.017$) & 0.474 & \textbf{0.509}   \\ \hline
NIPS & 0.379 ($\pm 0.01$) & \textbf{0.415} ($\pm 0.037$) & \textbf{0.396} ($\pm 0.022$) & 0.39($\pm 0.018$) & 0.384 ($\pm 0.014$) & \textbf{0.407} ($\pm 0.031$) & 0.466 & \textbf{0.503}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.517 ($\pm 0.044$) & \textbf{0.528} ($\pm 0.043$) & 0.322 ($\pm 0.024$) & \textbf{0.401} ($\pm 0.026$) & 0.516 ($\pm 0.037$) & \textbf{0.525} ($\pm 0.037$) & 0.403 & \textbf{0.427}   \\ \hline
Reuters & 0.324 ($\pm 0.029$) & \textbf{0.363} ($\pm 0.032$) & 0.222 ($\pm 0.011$) & \textbf{0.282} ($\pm 0.02$) & 0.339 ($\pm 0.023$) & \textbf{0.378} ($\pm 0.024$) & 0.277 & \textbf{0.339}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.292} ($\pm 0.015$) & 0.289($\pm 0.014$) & 0.383 ($\pm 0.009$) & \textbf{0.387} ($\pm 0.01$) & \textbf{0.298} ($\pm 0.017$) & 0.297($\pm 0.017$) & \textbf{0.285} & 0.276 \\ \hline
RCV1 & 0.243 ($\pm 0.008$) & \textbf{0.247} ($\pm 0.008$) & 0.279 ($\pm 0.01$) & \textbf{0.295} ($\pm 0.011$) & 0.242 ($\pm 0.01$) & \textbf{0.245} ($\pm 0.011$) & 0.239 & \textbf{0.24}   \\ \hline
PIE-Expr & 0.81 ($\pm 0.021$) & \textbf{0.85} ($\pm 0.019$) & 0.783 ($\pm 0.023$) & \textbf{0.809} ($\pm 0.024$) & 0.617 ($\pm 0.019$) & \textbf{0.7} ($\pm 0.02$) & \textbf{0.536} & 0.513 \\ \hline
ORL & 0.776 ($\pm 0.017$) & \textbf{0.811} ($\pm 0.018$) & 0.465 ($\pm 0.019$) & \textbf{0.608} ($\pm 0.026$) & 0.77 ($\pm 0.013$) & \textbf{0.804} ($\pm 0.015$) & 0.653 & \textbf{0.71}   \\ \hline
COIL-20 & 0.727 ($\pm 0.036$) & \textbf{0.729} ($\pm 0.037$) & 0.478 ($\pm 0.023$) & \textbf{0.507} ($\pm 0.025$) & 0.739 ($\pm 0.046$) & \textbf{0.741} ($\pm 0.046$) & \textbf{0.674} & 0.672 \\ \hline
ExtYaleB & \textbf{0.235} ($\pm 0.008$) & 0.228($\pm 0.007$) & 0.194 ($\pm 0.007$) & \textbf{0.197} ($\pm 0.009$) & \textbf{0.237} ($\pm 0.012$) & 0.23($\pm 0.01$) & 0.229 & \textbf{0.242}   \\ \hline
 \end{tabular}
 \end{table*}


==> performance_sv_100_floor_log.tex <==
\begin{table*}[tb] \centering \label{tab:results} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.464 ($\pm 0.017$) & \textbf{0.49} ($\pm 0.019$) & 0.429 ($\pm 0.022$) & \textbf{0.434} ($\pm 0.02$) & 0.467 ($\pm 0.013$) & \textbf{0.495} ($\pm 0.014$) & 0.474 & \textbf{0.509}   \\ \hline
NIPS & 0.381 ($\pm 0.012$) & \textbf{0.409} ($\pm 0.032$) & \textbf{0.4} ($\pm 0.015$) & 0.39($\pm 0.011$) & 0.38 ($\pm 0.013$) & \textbf{0.403} ($\pm 0.034$) & 0.466 & \textbf{0.506}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.522 ($\pm 0.049$) & \textbf{0.531} ($\pm 0.051$) & 0.339 ($\pm 0.033$) & \textbf{0.408} ($\pm 0.032$) & 0.502 ($\pm 0.058$) & \textbf{0.514} ($\pm 0.052$) & 0.403 & \textbf{0.427}   \\ \hline
Reuters & 0.33 ($\pm 0.021$) & \textbf{0.367} ($\pm 0.021$) & 0.222 ($\pm 0.008$) & \textbf{0.28} ($\pm 0.015$) & 0.341 ($\pm 0.018$) & \textbf{0.377} ($\pm 0.02$) & 0.277 & \textbf{0.333}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.294} ($\pm 0.014$) & 0.291($\pm 0.014$) & 0.384 ($\pm 0.012$) & \textbf{0.387} ($\pm 0.013$) & \textbf{0.297} ($\pm 0.012$) & 0.296($\pm 0.012$) & \textbf{0.285} & 0.276 \\ \hline
PIE-Expr & 0.809 ($\pm 0.027$) & \textbf{0.849} ($\pm 0.025$) & 0.791 ($\pm 0.02$) & \textbf{0.81} ($\pm 0.023$) & 0.622 ($\pm 0.018$) & \textbf{0.697} ($\pm 0.025$) & \textbf{0.536} & 0.53 \\ \hline
ORL & 0.775 ($\pm 0.017$) & \textbf{0.802} ($\pm 0.015$) & 0.456 ($\pm 0.019$) & \textbf{0.59} ($\pm 0.022$) & 0.776 ($\pm 0.015$) & \textbf{0.801} ($\pm 0.017$) & 0.653 & \textbf{0.735}   \\ \hline
COIL-20 & 0.716 ($\pm 0.052$) & \textbf{0.72} ($\pm 0.052$) & 0.476 ($\pm 0.028$) & \textbf{0.497} ($\pm 0.027$) & 0.745 ($\pm 0.046$) & \textbf{0.749} ($\pm 0.047$) & 0.669 & \textbf{0.671}   \\ \hline
ExtYaleB & \textbf{0.237} ($\pm 0.013$) & 0.231($\pm 0.011$) & 0.195 ($\pm 0.008$) & \textbf{0.202} ($\pm 0.009$) & \textbf{0.238} ($\pm 0.01$) & 0.232($\pm 0.009$) & 0.229 & \textbf{0.239}   \\ \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.386 ($\pm 0.012$) & \textbf{0.402} ($\pm 0.012$) & 0.374 ($\pm 0.026$) & \textbf{0.398} ($\pm 0.016$) & 0.388 ($\pm 0.006$) & \textbf{0.405} ($\pm 0.011$) & 0.388 & \textbf{0.401}   \\ \hline
NIPS & 0.389 ($\pm 0.009$) & \textbf{0.407} ($\pm 0.009$) & 0.404 ($\pm 0.015$) & \textbf{0.411} ($\pm 0.012$) & 0.388 ($\pm 0.009$) & \textbf{0.403} ($\pm 0.013$) & 0.388 & \textbf{0.418}   \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.499 ($\pm 0.017$) & \textbf{0.506} ($\pm 0.019$) & 0.456 ($\pm 0.02$) & \textbf{0.494} ($\pm 0.016$) & 0.495 ($\pm 0.019$) & \textbf{0.501} ($\pm 0.018$) & \textbf{0.427} & 0.426 \\ \hline
Reuters & 0.518 ($\pm 0.006$) & \textbf{0.525} ($\pm 0.005$) & 0.442 ($\pm 0.006$) & \textbf{0.493} ($\pm 0.004$) & 0.52 ($\pm 0.007$) & \textbf{0.527} ($\pm 0.006$) & 0.488 & \textbf{0.491}   \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 ($\pm 0.01$) & \textbf{0.421} ($\pm 0.01$) & 0.511 ($\pm 0.006$) & \textbf{0.517} ($\pm 0.006$) & 0.404 ($\pm 0.012$) & \textbf{0.419} ($\pm 0.011$) & \textbf{0.403} & 0.402 \\ \hline
PIE-Expr & 0.951 ($\pm 0.007$) & \textbf{0.967} ($\pm 0.005$) & 0.941 ($\pm 0.007$) & \textbf{0.961} ($\pm 0.005$) & 0.889 ($\pm 0.005$) & \textbf{0.932} ($\pm 0.006$) & 0.861 & \textbf{0.894}   \\ \hline
ORL & 0.889 ($\pm 0.007$) & \textbf{0.914} ($\pm 0.004$) & 0.682 ($\pm 0.017$) & \textbf{0.833} ($\pm 0.014$) & 0.89 ($\pm 0.005$) & \textbf{0.914} ($\pm 0.005$) & 0.808 & \textbf{0.889}   \\ \hline
COIL-20 & 0.87 ($\pm 0.015$) & \textbf{0.875} ($\pm 0.016$) & 0.62 ($\pm 0.017$) & \textbf{0.663} ($\pm 0.015$) & 0.878 ($\pm 0.009$) & \textbf{0.884} ($\pm 0.011$) & 0.82 & \textbf{0.835}   \\ \hline
ExtYaleB & 0.306 ($\pm 0.008$) & \textbf{0.315} ($\pm 0.006$) & 0.356 ($\pm 0.008$) & \textbf{0.365} ($\pm 0.008$) & 0.311 ($\pm 0.008$) & \textbf{0.319} ($\pm 0.005$) & 0.288 & \textbf{0.314}   \\ \hline
 \end{tabular}
 \caption{Performance of the GT-NMF compared to other approaches.}
 \end{table*}


==> performance_sv_100_sv_floor_log.tex <==
\begin{table*}[tb] \centering \label{tab:results} \begin{tabular}{|l|c|c|c|c|c|c|c|c|} \hline
 \multicolumn{9}{c}{\textbf{Accuracy}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.464 & \textbf{0.49} (+2.6\%) & 0.429 & \textbf{0.434} (+0.5\%) & 0.467 & \textbf{0.495} (+2.8\%) & 0.474 & \textbf{0.509} (+3.5\%) \\ \hline
NIPS & 0.381 & \textbf{0.409} (+2.8\%) & \textbf{0.4} & 0.39(--1\%) & 0.38 & \textbf{0.403} (+2.3\%) & 0.466 & \textbf{0.506} (+4\%) \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.522 & \textbf{0.531} (+0.9\%) & 0.339 & \textbf{0.408} (+6.9\%) & 0.502 & \textbf{0.514} (+1.2\%) & 0.403 & \textbf{0.427} (+2.4\%) \\ \hline
Reuters & 0.33 & \textbf{0.367} (+3.7\%) & 0.222 & \textbf{0.28} (+5.8\%) & 0.341 & \textbf{0.377} (+3.6\%) & 0.277 & \textbf{0.333} (+5.6\%) \\ \hline
RCV1 \textsuperscript{$\bigstar$} & \textbf{0.294} & 0.291(--0.3\%) & 0.384 & \textbf{0.387} (+0.3\%) & \textbf{0.297} & 0.296(--0.1\%) & \textbf{0.285} & 0.276(--0.9\%) \\ \hline
PIE-Expr & 0.809 & \textbf{0.849} (+4\%) & 0.791 & \textbf{0.81} (+1.9\%) & 0.622 & \textbf{0.697} (+7.5\%) & \textbf{0.536} & 0.53(--0.6\%) \\ \hline
ORL & 0.775 & \textbf{0.802} (+2.7\%) & 0.456 & \textbf{0.59} (+13.4\%) & 0.776 & \textbf{0.801} (+2.5\%) & 0.653 & \textbf{0.735} (+8.2\%) \\ \hline
COIL-20 & 0.716 & \textbf{0.72} (+0.4\%) & 0.476 & \textbf{0.497} (+2.1\%) & 0.745 & \textbf{0.749} (+0.4\%) & 0.669 & \textbf{0.671} (+0.2\%) \\ \hline
ExtYaleB & \textbf{0.237} & 0.231(--0.6\%) & 0.195 & \textbf{0.202} (+0.7\%) & \textbf{0.238} & 0.232(--0.6\%) & 0.229 & \textbf{0.239} (+1\%) \\ \hline
 \multicolumn{9}{c}{\textbf{Normalized Mutual Information}} \\ \hline
Dataset & SymNMF & SymNMF+GT & NMF\footnote{Implementation at: https://github.com/kimjingu/nonnegfac-matlab} & NMF+GT &  NMFS &  NMFS+GT & NNDSVD & NNDSVD+GT \\ \hline
NIPS \textsuperscript{$\bigstar$} & 0.386 & \textbf{0.402} (+1.6\%) & 0.374 & \textbf{0.398} (+2.4\%) & 0.388 & \textbf{0.405} (+1.7\%) & 0.388 & \textbf{0.401} (+1.3\%) \\ \hline
NIPS & 0.389 & \textbf{0.407} (+1.8\%) & 0.404 & \textbf{0.411} (+0.7\%) & 0.388 & \textbf{0.403} (+1.5\%) & 0.388 & \textbf{0.418} (+3\%) \\ \hline
Reuters \textsuperscript{$\bigstar$} & 0.499 & \textbf{0.506} (+0.7\%) & 0.456 & \textbf{0.494} (+3.8\%) & 0.495 & \textbf{0.501} (+0.6\%) & \textbf{0.427} & 0.426(--0.1\%) \\ \hline
Reuters & 0.518 & \textbf{0.525} (+0.7\%) & 0.442 & \textbf{0.493} (+5.1\%) & 0.52 & \textbf{0.527} (+0.7\%) & 0.488 & \textbf{0.491} (+0.3\%) \\ \hline
RCV1 \textsuperscript{$\bigstar$} & 0.406 & \textbf{0.421} (+1.5\%) & 0.511 & \textbf{0.517} (+0.6\%) & 0.404 & \textbf{0.419} (+1.5\%) & \textbf{0.403} & 0.402(--0.1\%) \\ \hline
PIE-Expr & 0.951 & \textbf{0.967} (+1.6\%) & 0.941 & \textbf{0.961} (+2\%) & 0.889 & \textbf{0.932} (+4.3\%) & 0.861 & \textbf{0.894} (+3.3\%) \\ \hline
ORL & 0.889 & \textbf{0.914} (+2.5\%) & 0.682 & \textbf{0.833} (+15.1\%) & 0.89 & \textbf{0.914} (+2.4\%) & 0.808 & \textbf{0.889} (+8.1\%) \\ \hline
COIL-20 & 0.87 & \textbf{0.875} (+0.5\%) & 0.62 & \textbf{0.663} (+4.3\%) & 0.878 & \textbf{0.884} (+0.6\%) & 0.82 & \textbf{0.835} (+1.5\%) \\ \hline
ExtYaleB & 0.306 & \textbf{0.315} (+0.9\%) & 0.356 & \textbf{0.365} (+0.9\%) & 0.311 & \textbf{0.319} (+0.8\%) & 0.288 & \textbf{0.314} (+2.6\%) \\ \hline
 \end{tabular}
 \caption{Performance at 100 iteration for SV Method. Mean Loss(-0.11389  -0.0055556) Mean Gain(2.6083      2.2472).}
 \end{table*}


==> seba.tex <==
%\section{Similarity Matrix construction}\label{sec:smc}
%
%The same pipeline of \cite{kuang2015symnmf} has been used to construct the similarity matrix, this has been done to fairly compare the performances at the end. Given a feature matrix of $n \times m$ data in which $n$ is the number of points and $m$ the size of the feature, each point became a vertex and the weight of the edges $e_{ij}$ are computed in the following 3 steps:\\
%
%\emph{1. Construct a complete graph}: If the dataset $X$ is textual each row is normalized to have unit 2-norm and $e_{i,j}={x_i}^Tx_j$ are the cosine distance of point $i$ and $j$. If $X$ is made of images each feature (column) is first normalized by its maximum value to lie in $[0,1]$ and then the weight are $e_{i,j}=\exp\{- \frac{||x_i-x_j||}{\sigma_i\sigma_j}\}$ where $\sigma_i=||x_i-\hat{x_i}||$ is a scaling parameter and $\hat{x_i}$ is the 7-th nearest neighbors, as suggested in \cite{Zelnik-manor04self-tuningspectral}. In all cases $e_{ii}=0$.\\
%
%\emph{2. Graph sparsification}: Only the edges connecting $q$ neighbors are kept. The parameter $q$ is set accordingly to \cite{Luxburg2007} $q=\floor{log_2(n)}+1$, let $N(i)=\{ j \mbox{ s.t. } x_j \in q\mbox{-NN of } i \}$. The weight on the edges are $\hat{e}_{ij}=e_{ij}$ if $i \in N(j) \mbox{ or } j\in N(i)$ and $\hat{e}_{ij}=0$ otherwise.\\
%
%\emph{3. Similarity Matrix}: the same normalization of normalized-cut has been applied on the sparse graph obtaining the final matrix $A_{ij}=\hat{e}_{ij}\sqrt{d_i}\sqrt{d_j}$ where $d_i=\sum_{s=1}^n{\hat{e}_{is}}$.
%



\section{Adaptive auto-tuning} When constructing the payoff matrix $A$ for the
game dynamics the same procedure of Sec \ref{sec:smc} is used with the only,
important, difference on how the parameter $q$ is chosen. The assumption here is
that the clustering results obtained via NMF provides a good insight on the size
of the final clusters and this information can be used to select the number of
$q$. The rationale is that clusters induces games in which the number of players
is in the order of the number of the elements within them (small clusters let a
small number of players to ply while bigger clusters let a bigger number of
players to play). In this context having a fixed $q$ all the clusters may lead
to have players belonging to small cluster that plays with a bigger number of
opponents. The idea to solve this problem by using the same idea of
\cite{Luxburg2007} applied in a local context having a variable $q$ for all
clusters obtained via NMF. Given a point $i$ and its clustering membership $C$
from NMF ($i \in C$), the number of neighbors used to construct the similarity
matrix is related to the expected number of points in the cluster $C$. This
results in having a variable number of expected number of neighbors depending on
the clusters size $q_i= \floor{log(|C|)}+1$ where $|C|$ is the cardinality of
cluster $C$. This intuition have the following combinatorial counterpart: a
theoretical bound to prove the connectedness of a graph \cite{Luxburg2007} is
that a graph is connected if the number of neighbors of each node is
$k=\floor{log(n)}+1$. A cluster $C$ can be considered as a fully connected
subgraph and thus connected. Thus the number of neighbors of each element in the
cluster $C$ should be $k_C=\floor{log(|C|)}+1$ where $|C|$ is the number of
elements in the cluster otherwise the subgraph is not connected and thus is not
a cluster. 

\subsection{results analysis} A global analysis on the results obtained by the
GTNMF shown the efficancy of using this approach to refine the partitions
obtained by NMF and derivate methods. Despite the different settings
(textual/image datasets) the algorithm is able improve the NMI performance in
33/36 cases with a maximum gain of $\simeq 15.3\%$ (which is quite impressive)
and a maximum loss of 0.2\%. In terms of ACC on 27/36 cases the method improve
on previous results with a maximum gain of 14.3\% and loss of 2.3\%. The mean
gain for both NMI and ACC is $2.68\%$ and $2.30\%$ while the mean loss is in the
order of $0.16\%$ for the ACC and $0.01\%$ in the NMI (see Table
\ref{tab:results}). An almost constant gain in the NMI means, in practice, that
the algorithm is able to correctly relocate the points in the right cluster
after the NMF clustering. This is quite a good results if the gain is related to
the size of the dataset, i.e. a gain of $+1.6\%$ in RCV1 means that 212 elements
has been moved. Giving a closer look on the results one can notice that in some
cases the ACC and the NMI have opposite behavior in the sense that when there is
a drop in the ACC a gain is achieved in the NMI, this is quite normal and is
explained by the fact that the NMI provides hints on how good the data are
partitioned while the ACC counts only the correct assignment (ESEMPIO TOY DI
ROCCO), the opposite is indeed true as well. Checking more carefully the case in
which the performances are lower (PIE-Expr with NNDSVD+GT) this happens mainly
because the clusters are a lot (68) while the data per cluster is not constant
and rolls between 3 and 4, a small change in this dataset dramatically impact
the global performance.\\




For those dataset in which 

Giving a closer look on when the looses occurs one can notice that this happen
in deeper analysis on when the losses occur
